A Theoretically Sound Upper Bound on the Triplet Loss for Improving the Efficiency of Deep Distance Metric Learning

We propose a method that substantially improves the efficiency of deep distance metric learning based on the optimization of the triplet loss function. One epoch of such training process based on a naive optimization of the triplet loss function has a run-time complexity O(N^3), where N is the number of training samples. Such optimization scales poorly, and the most common approach proposed to address this high complexity issue is based on sub-sampling the set of triplets needed for the training process. Another approach explored in the field relies on an ad-hoc linearization (in terms of N) of the triplet loss that introduces class centroids, which must be optimized using the whole training set for each mini-batch - this means that a naive implementation of this approach has run-time complexity O(N^2). This complexity issue is usually mitigated with poor, but computationally cheap, approximate centroid optimization methods. In this paper, we first propose a solid theory on the linearization of the triplet loss with the use of class centroids, where the main conclusion is that our new linear loss represents a tight upper-bound to the triplet loss. Furthermore, based on the theory above, we propose a training algorithm that no longer requires the centroid optimization step, which means that our approach is the first in the field with a guaranteed linear run-time complexity. We show that the training of deep distance metric learning methods using the proposed upper-bound is substantially faster than triplet-based methods, while producing competitive retrieval accuracy results on benchmark datasets (CUB-200-2011 and CAR196).

==> improve-vgg.tex <==
\subsection{Improving with Different Network Architectures}
In this section we present improved results when using the proposed discriminative loss with other network architectures. \gustavo{we need to mention: 7) Gradient Analysis (ICLR 2019 submission) : achieves 66.85 and 83.69 for CUB and CARS respectively (Uses Inception v2)
8) Deep Randomized Ensemble Metric Learning (ECCV 2018) : achieves 78.5 (80.5) and 89.8 (86) for CUB and CARS respectively [Uses Inception v3(Resnet-18)]
9) DML with Heirarchical Triplet loss (ECCV 2018) : achieves 57.1 and 81.4 for CUB and CARS respectively (Uses Inception v2)
10) Sampling matters (ICCV 2017) :achieves 63.6 and 79.6 for CUB and CARS respectively (Uses Resnet-50).}

\subsubsection{Maximum Activations of Convolution Layer}
In GoogleNet~\cite{googlenet} which is trained for the image classification task, the authors applied an average pooling on the activations of the last convolutional layer to produce a single representation which has 1024 dimensions. Recently, in~\cite{DBLP:journals/corr/ToliasSJ15}, the authors showed that applying max-pooling on the CNN activations (referred to as MAC layer) of one of the last convolutional layers will produce more discriminative feature representations for new tasks such as object instance retrieval. In this section, we test if the use of MAC features is advantageous in the DML problem, where we replace the last average pooling layer of GoogleNet by the MAC layer. 
Table~\ref{tab:mac} shows the results when using MAC layer in the GoogleNet. From Tables~\ref{tab:cub},~\ref{tab:car} and~\ref{tab:mac}, we can see that using MAC layer provides competitive or better performance than the average layer on both CUB-200-2011 and CAR196 datasets, e.g., on the CAR196 dataset, using the MAC layer improves the recall from 1\% to 2.4\% at different $K$ values. We note that both average pooling and max pooling has the same computational complexity, so using MAC layer does not increase the complexity in both training and test stages. 

\begin{table}
\footnotesize
\centering
 \begin{center}
\begin{tabular}{c c c c c c}
\hline
		 		&NMI &R@1 &R@2 &R@4 &R@8 \\ \hline
CUB-200-2011    &59.96 &52.31 &64.11 &74.83 &84.23  \\ \hline
CAR196 			&58.80 &70.71 &80.36 &87.23 &92.22 \\ \hline
\end{tabular}
\end{center}
\caption{Clustering and recall performance when using Maximum Activations of Convolution Layer~\cite{DBLP:journals/corr/ToliasSJ15} for the GoogleNet with discriminative loss.}
\label{tab:mac}
\end{table}

\subsubsection{VGG network}
As presented in Section~\ref{subsec:diss}, the proposed discriminative loss is simple and it is easy to integrate into any deep learning models. In this section we experiment the proposed loss with the VGG-16 network~\cite{vgg}. We also add a MAC layer after the last convolutional layer of VGG for producing a 512-D feature representation. After that, similarly to GoogleNet in Section~\ref{subsec:architecture}, we add two fully connected layers whose dimensions are $256$ and $C$. The outputs of the second to last layer are used as embedding features. Table~\ref{tab:vgg} presents the results when using our discriminative loss with VGG network. To the best of our knowledge, those results are the state of the art for DML on CUB-200-2011 and CAR196 datasets.
From Tables~\ref{tab:cub},~\ref{tab:car} and~\ref{tab:vgg}, we can see that using discriminative loss with VGG network significantly boosts the performance on both datasets, e.g., at $R@1$, it improves over GoogleNet $6.3\%$ and $9.8\%$ for CUB-200-2011 and CAR196, respectively. 
 
\begin{table}
\footnotesize
\centering
 \begin{center}
\begin{tabular}{c c c c c c}
\hline
		 		&NMI &R@1 &R@2 &R@4 &R@8 \\ \hline
CUB-200-2011    &61.49 &57.74 &68.46 &78.07 &85.40  \\ \hline
CAR196 			&62.14 &78.15 &85.70 &90.71 &94.21 \\ \hline
\end{tabular}
\end{center}
\caption{Clustering and recall performance when using VGG-16 network with discriminative loss.}
\label{tab:vgg}
\end{table}

